Modelling charge transport in gold nanogranular films

Cluster-assembled metallic films show interesting electrical properties, both in the near-to-percolation regime, when deposited clusters do not form a complete layer yet, and when the film thickness is well above the electrical percolation threshold. Correctly estimating their electrical conductivity is crucial, but, particularly for the latter regime, standard theoretical tools are not quite adequate. We therefore developed a procedure based on an atomically informed mesoscopic model in which ab-initio estimates of electronic transport at the nanoscale are used to reconstruct the conductivity of nanogranular gold films generated by molecular dynamics. An equivalent resistor network is developed, appropriately accounting for ballistic transport. The method is shown to correctly capture the non-monotonic behavior of the conductivity as a function of the film thickness, namely a signature feature of nanogranular films.

==> bibliography.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% GRANECO 2019 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{kawamura1993quantum,
  title={Quantum ballistic transport through a double-bend waveguide structure: Effects of disorder},
  author={Kawamura, T and Leburton, JP},
  journal={Physical Review B},
  volume={48},
  number={12},
  pages={8857},
  year={1993},
  publisher={APS}
}

@article{benetti2017,
author = {Benetti, Giulio and Caddeo, Claudia and Melis, Claudio and Ferrini, Gabriele and Giannetti, Claudio and Winckelmans, Naomi and Bals, Sara and Van Bael, Margriet J. and Cavaliere, Emanuele and Gavioli, Luca and Banfi, Francesco},
title = {Bottom-Up Mechanical Nanometrology of Granular Ag Nanoparticles Thin Films},
journal = {The Journal of Physical Chemistry C},
volume = {121},
number = {40},
pages = {22434-22441},
year = {2017},
doi = {10.1021/acs.jpcc.7b05795},

URL = { 
        https://doi.org/10.1021/acs.jpcc.7b05795
    
},
eprint = { 
        https://doi.org/10.1021/acs.jpcc.7b05795
    
}

}

@ARTICLE{7878935,  author={Theis, Thomas N. and Wong, H.-S. Philip},  journal={Computing in Science   Engineering},   title={The End of Moore's Law: A New Beginning for Information Technology},   year={2017},  volume={19},  number={2},  pages={41-50},  doi={10.1109/MCSE.2017.29}}

@article{diventra2018,
author = {Di Ventra,Massimiliano  and Traversa,Fabio L. },
title = {Perspective: Memcomputing: Leveraging memory and physics to compute efficiently},
journal = {Journal of Applied Physics},
volume = {123},
number = {18},
pages = {180901},
year = {2018},
doi = {10.1063/1.5026506},

URL = { 
        https://doi.org/10.1063/1.5026506
    
},
eprint = { 
        https://doi.org/10.1063/1.5026506
    
}

}
@ARTICLE{7549034,  author={Nawrocki, Robert A. and Voyles, Richard M. and Shaheen, Sean E.},  journal={IEEE Transactions on Electron Devices},   title={A Mini Review of Neuromorphic Architectures and Implementations},   year={2016},  volume={63},  number={10},  pages={3819-3829},  doi={10.1109/TED.2016.2598413}}

@Article{ielmini2018,
author={Ielmini, Daniele
and Wong, H.-S. Philip},
title={In-memory computing with resistive switching devices},
journal={Nature Electronics},
year={2018},
month={Jun},
day={01},
volume={1},
number={6},
pages={333-343},
abstract={Modern computers are based on the von Neumann architecture in which computation and storage are physically separated: data are fetched from the memory unit, shuttled to the processing unit (where computation takes place) and then shuttled back to the memory unit to be stored. The rate at which data can be transferred between the processing unit and the memory unit represents a fundamental limitation of modern computers, known as the memory wall. In-memory computing is an approach that attempts to address this issue by designing systems that compute within the memory, thus eliminating the energy-intensive and time-consuming data movement that plagues current designs. Here we review the development of in-memory computing using resistive switching devices, where the two-terminal structure of the devices, their resistive switching properties, and direct data processing in the memory can enable area- and energy-efficient computation. We examine the different digital, analogue, and stochastic computing schemes that have been proposed, and explore the microscopic physical mechanisms involved. Finally, we discuss the challenges in-memory computing faces, including the required scaling characteristics, in delivering next-generation computing.},
issn={2520-1131},
doi={10.1038/s41928-018-0092-2},
url={https://doi.org/10.1038/s41928-018-0092-2}
}
@misc{HadaeghiHeJaeger2017,
  author    = {Fatemeh Hadaeghi and Xu He and Herbert Jaeger},
  title     = {Unconventional Information Processing Systems, Novel Hardware: A Tour d'Horizon},
  series    = {Jacobs University Technical Reports},
  number    = {36},
  year        = {2017},
}


@ARTICLE{traversa2015,  author={Traversa, Fabio Lorenzo and Di Ventra, Massimiliano},  journal={IEEE Transactions on Neural Networks and Learning Systems},   title={Universal Memcomputing Machines},   year={2015},  volume={26},  number={11},  pages={2702-2715},  doi={10.1109/TNNLS.2015.2391182}}
@article{soler2002siesta,
  title={The SIESTA method for ab initio order-N materials simulation},
  author={Soler, Jos{\'e} M and Artacho, Emilio and Gale, Julian D and Garc{\'\i}a, Alberto and Junquera, Javier and Ordej{\'o}n, Pablo and S{\'a}nchez-Portal, Daniel},
  journal={Journal of Physics: Condensed Matter},
  volume={14},
  number={11},
  pages={2745},
  year={2002},
  publisher={IOP Publishing}
}

@article{brandbyge2002density,
  title={Density-functional method for nonequilibrium electron transport},
  author={Brandbyge, Mads and Mozos, Jos{\'e}-Luis and Ordej{\'o}n, Pablo and Taylor, Jeremy and Stokbro, Kurt},
  journal={Physical Review B},
  volume={65},
  number={16},
  pages={165401},
  year={2002},
  publisher={APS}
}

@article{kurui2009conductance,
  title={Conductance quantization and dequantization in gold nanowires due to multiple reflection at the interface},
  author={Kurui, Yoshihiko and Oshima, Yoshifumi and Okamoto, Masakuni and Takayanagi, Kunio},
  journal={Physical Review B},
  volume={79},
  number={16},
  pages={165414},
  year={2009},
  publisher={APS}
}

@article{kizuka2008atomic,
  title={Atomic configuration and mechanical and electrical properties of stable gold wires of single-atom width},
  author={Kizuka, Tokushi},
  journal={Physical review B},
  volume={77},
  number={15},
  pages={155401},
  year={2008},
  publisher={APS}
}

@article{erts2000maxwell,
  title={Maxwell and Sharvin conductance in gold point contacts investigated using TEM-STM},
  author={Erts, D and Olin, H{\aa}kan and Ryen, L and Olsson, E and Th{\"o}l{\'e}n, A},
  journal={Physical Review B},
  volume={61},
  number={19},
  pages={12725},
  year={2000},
  publisher={APS}
}

@article{yasuda1997conductance,
  title={Conductance of atomic-scale gold contacts under high-bias voltages},
  author={Yasuda, Hiroshi and Sakai, Akira},
  journal={Physical Review B},
  volume={56},
  number={3},
  pages={1069},
  year={1997},
  publisher={APS}
}

@article{tavazza2011electron,
  title={Electron transport in gold nanowires: Stable 1-, 2-and 3-dimensional atomic structures and noninteger conduction states},
  author={Tavazza, F and Smith, Douglas T and Levine, Lyle E and Pratt, Jon R and Chaka, Anne M},
  journal={Physical review letters},
  volume={107},
  number={12},
  pages={126802},
  year={2011},
  publisher={APS}
}

@article{suzuki2007distribution,
  title={Distribution of 1G0 plateau length of Au contacts at room temperature},
  author={Suzuki, Ryo and Tsutsui, Makusu and Miura, Daisuke and Kurokawa, Shu and Sakai, Akira},
  journal={Japanese journal of applied physics},
  volume={46},
  number={6R},
  pages={3694},
  year={2007},
  publisher={IOP Publishing}
}

@article{kiguchi2006conductance,
  title={Conductance bistability of gold nanowires at room temperature},
  author={Kiguchi, Manabu and Konishi, Tatsuya and Murakoshi, Kei},
  journal={Physical Review B},
  volume={73},
  number={12},
  pages={125406},
  year={2006},
  publisher={APS}
}

@article{neel2007controlled,
  title={Controlled contact to a C 60 molecule},
  author={N{\'e}el, N and Kr{\"o}ger, J and Limot, L and Frederiksen, Thomas and Brandbyge, Mads and Berndt, R},
  journal={Physical review letters},
  volume={98},
  number={6},
  pages={065502},
  year={2007},
  publisher={APS}
}

@article{dai2005effects,
  title={Effects of contact geometry on transport properties of a Si 4 cluster},
  author={Dai, ZX and Zheng, XH and Shi, XQ and Zeng, Z},
  journal={Physical Review B},
  volume={72},
  number={20},
  pages={205408},
  year={2005},
  publisher={APS}
}

@article{oshima2003development,
  title={Development of a miniature STM holder for study of electronic conductance of metal nanowires in UHV--TEM},
  author={Oshima, Y and Mouri, K and Hirayama, H and Takayanagi, K},
  journal={Surface science},
  volume={531},
  number={3},
  pages={209--216},
  year={2003},
  publisher={Elsevier}
}

@article{rodrigues2000signature,
  title={Signature of atomic structure in the quantum conductance of gold nanowires},
  author={Rodrigues, Varlei and Fuhrer, Tobias and Ugarte, Daniel},
  journal={Physical review letters},
  volume={85},
  number={19},
  pages={4124},
  year={2000},
  publisher={APS}
}

@article{dreher2005structure,
  title={Structure and conductance histogram of atomic-sized Au contacts},
  author={Dreher, Markus and Pauly, Fabian and Heurich, Jan and Cuevas, Juan Carlos and Scheer, Elke and Nielaba, Peter},
  journal={Physical Review B},
  volume={72},
  number={7},
  pages={075435},
  year={2005},
  publisher={APS}
}

@article{yanson2005atomic,
  title={Atomic-size oscillations in conductance histograms for gold nanowires and the influence of work hardening},
  author={Yanson, IK and Shklyarevskii, OI and Csonka, Sz and Van Kempen, H and Speller, S and Yanson, AI and Van Ruitenbeek, JM},
  journal={Physical review letters},
  volume={95},
  number={25},
  pages={256806},
  year={2005},
  publisher={APS}
}

@article{ohno2011short,
  title={Short-term plasticity and long-term potentiation mimicked in single inorganic synapses},
  author={Ohno, Takeo and Hasegawa, Tsuyoshi and Tsuruoka, Tohru and Terabe, Kazuya and Gimzewski, James K and Aono, Masakazu},
  journal={Nature materials},
  volume={10},
  number={8},
  pages={591--595},
  year={2011},
  publisher={Nature Publishing Group}
}

@article{bose2019synaptic,
  title={Synaptic dynamics in complex self-assembled nanoparticle networks},
  author={Bose, SK and Shirai, S and Mallinson, JB and Brown, SA},
  journal={Faraday discussions},
  volume={213},
  pages={471--485},
  year={2019},
  publisher={The Royal Society of Chemistry}
}

@article{lee2015resistive,
  title={Resistive switching phenomena: A review of statistical physics approaches},
  author={Lee, Jae Sung and Lee, Shinbuhm and Noh, Tae Won},
  journal={Applied Physics Reviews},
  volume={2},
  number={3},
  pages={031303},
  year={2015},
  publisher={AIP Publishing LLC}
}

@article{minnai2017facile,
  title={Facile fabrication of complex networks of memristive devices},
  author={Minnai, Chlo{\'e} and Bellacicca, Andrea and Brown, Simon A and Milani, Paolo},
  journal={Scientific reports},
  volume={7},
  number={1},
  pages={1--8},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{avizienis2012neuromorphic,
  title={Neuromorphic atomic switch networks},
  author={Avizienis, Audrius V and Sillin, Henry O and Martin-Olmos, Cristina and Shieh, Hsien Hang and Aono, Masakazu and Stieg, Adam Z and Gimzewski, James K},
  journal={PloS one},
  volume={7},
  number={8},
  pages={e42772},
  year={2012},
  publisher={Public Library of Science}
}

@Article{mirigliano2019,
author ="Mirigliano, M. and Borghi, F. and Podestà, A. and Antidormi, A. and Colombo, L. and Milani, P.",
title  ="Non-ohmic behavior and resistive switching of Au cluster-assembled films beyond the percolation threshold",
journal  ="Nanoscale Adv.",
year  ="2019",
volume  ="1",
issue  ="8",
pages  ="3119-3130",
publisher  ="RSC",
doi  ="10.1039/C9NA00256A",
url  ="http://dx.doi.org/10.1039/C9NA00256A"
}

@article{barborini2010influence,
  title={The influence of nanoscale morphology on the resistivity of cluster-assembled nanostructured metallic thin films},
  author={Barborini, E and Corbelli, G and Bertolini, G and Repetto, P and Leccardi, M and Vinati, S and Milani, P},
  journal={New Journal of Physics},
  volume={12},
  number={7},
  pages={073001},
  year={2010},
  publisher={IOP Publishing}
}

@article{landauer1989conductance,
  title={Conductance determined by transmission: probes and quantised constriction resistance},
  author={Landauer, Rolf},
  journal={Journal of Physics: Condensed Matter},
  volume={1},
  number={43},
  pages={8099},
  year={1989},
  publisher={IOP Publishing}
}

@article{stukowski2009visualization,
  title={Visualization and analysis of atomistic simulation data with OVITO--the Open Visualization Tool},
  author={Stukowski, Alexander},
  journal={Modelling and Simulation in Materials Science and Engineering},
  volume={18},
  number={1},
  pages={015012},
  year={2009},
  publisher={IOP Publishing}
}

@Article{hebard1999,
author={Hebard, A. F.
and Arnason, S. B.},
title={Bad-Metal Behavior: Exotic Physics or a Consequence of Microstructure?},
journal={Journal of Superconductivity},
year={1999},
month={Feb},
day={01},
volume={12},
number={1},
pages={159-162},
abstract={A geometric renormalization associated with microstructure in coalescing silver films is shown to be responsible for metallic behavior on anomalously high resistivity scales. The signature for this effect, a proportional enhancement of residual resistivity and the temperature slope, may help determine the relevance of microstructure to other ``band metal'' systems.},
issn={1572-9605},
doi={10.1023/A:1007714813001},
url={https://doi.org/10.1023/A:1007714813001}
}



@Inbook{gould2017,
author="Gould, Robert D.
and Kasap, Safa
and Ray, Asim K.",
editor="Kasap, Safa
and Capper, Peter",
title="Thin Films",
bookTitle="Springer Handbook of Electronic and Photonic Materials",
year="2017",
publisher="Springer International Publishing",
address="Cham",
pages="1--1",
abstract="This chapter provides an extended introduction to the basic principles of thin-film technologythin filmtechnology, including deposition processes, structure, and some optical and electrical properties relevant to this volume. The material is accessible to scientists and engineers with no previous experience in this field, and contains extensive references to both the primary literature and earlier review articles. Although it is impossible to provide full coverage of all areas or of the most recent developments in this survey, references are included to enable the reader to access the information elsewhere, while the coverage of fundamentals will allow this to be appreciated.",
isbn="978-3-319-48933-9",
doi="10.1007/978-3-319-48933-9_28",
url="https://doi.org/10.1007/978-3-319-48933-9_28"
}

@article{neel2007controlled,
  title={Controlled contact to a C 60 molecule},
  author={N{\'e}el, N and Kr{\"o}ger, J and Limot, L and Frederiksen, Thomas and Brandbyge, Mads and Berndt, R},
  journal={Physical review letters},
  volume={98},
  number={6},
  pages={065502},
  year={2007},
  publisher={APS}
}

@article{torquato2018,
author = {Torquato,S. },
title = {Perspective: Basic understanding of condensed phases of matter via packing models},
journal = {The Journal of Chemical Physics},
volume = {149},
number = {2},
pages = {020901},
year = {2018},
doi = {10.1063/1.5036657},

URL = {
        https://doi.org/10.1063/1.5036657

},
eprint = {
        https://doi.org/10.1063/1.5036657
}
}

@article{chaudhuri2010,
  title = {Jamming Transitions in Amorphous Packings of Frictionless Spheres Occur over a Continuous Range of Volume Fractions},
  author = {Chaudhuri, Pinaki and Berthier, Ludovic and Sastry, Srikanth},
  journal = {Phys. Rev. Lett.},
  volume = {104},
  issue = {16},
  pages = {165701},
  numpages = {4},
  year = {2010},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.104.165701},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.104.165701}
}
@Article{landauer1978,
author={Landauer,Rolf},
title={Electrical conductivity in inhomogeneous media},
journal={AIP Conference Proceedings},
year={1978},
volume={40},
number={1},
pages={2-45},
abstract={ },
doi={10.1063/1.31150},
url={https://aip.scitation.org/doi/abs/10.1063/1.31150}
}

@article{gall2016electron,
  title={Electron mean free path in elemental metals},
  author={Gall, Daniel},
  journal={Journal of Applied Physics},
  volume={119},
  number={8},
  pages={085101},
  year={2016},
  publisher={AIP Publishing LLC}
}

@article{sheng1992electronic,
  title={Electronic transport in granular metal films},
  author={Sheng, Ping},
  journal={Philosophical Magazine B},
  volume={65},
  number={3},
  pages={357--384},
  year={1992},
  publisher={Taylor \& Francis}
}

@article{burgmann2005electrical,
  title={Electrical conductivity as a measure of the continuity of titanium and vanadium thin films},
  author={Burgmann, FA and Lim, SHN and McCulloch, DG and Gan, BK and Davies, KE and McKenzie, David Robert and Bilek, MMM},
  journal={Thin Solid Films},
  volume={474},
  number={1-2},
  pages={341--345},
  year={2005},
  publisher={Elsevier}
}

@article{maaroof1994onset,
  title={Onset of electrical conduction in Pt and Ni films},
  author={Maaroof, AI and Evans, BL},
  journal={Journal of applied Physics},
  volume={76},
  number={2},
  pages={1047--1054},
  year={1994},
  publisher={American Institute of Physics}
}

@article{kishore1992,
author = {Mohanty, Kishore K.},
title = {Porous media: Fluid transport and pore structure},
journal = {AIChE Journal},
volume = {38},
number = {8},
pages = {1303-1304},
year = {1992},
doi = {10.1002/aic.690380819},
URL = {https://aiche.onlinelibrary.wiley.com/doi/abs/10.1002/aic.690380819}
}




@article{maxwellgarnet1904,
author = {Garnett, J. C. M.},
title = {Colours in metal glasses and in metallic films},
journal = {Philos. Trans. R. Soc. London, Series A},
volume = {203},
number = {},
pages = {385-420},
year = {1904},
doi = {10.1002/10.1098/rsta.1904.0024},
URL = {https://royalsocietypublishing.org/doi/10.1098/rsta.1904.0024}
}

@article{bruggeman1935,
author = {Bruggeman, D. A. G.},
title = {Berechnung verschiedener physikalischer Konstanten von heterogenen Substanzen. I. Dielektrizitätskonstanten und Leitfähigkeiten der Mischkörper aus isotropen Substanzen},
journal = {Annalen der Physik},
volume = {416},
number = {7},
pages = {636-664},
doi = {10.1002/andp.19354160705},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/andp.19354160705},
abstract = {Abstract Es werden verschiedene physikalische Konstanten heterogener Körper aus den Konstanten ihrer homogenen Bestandteile nach einer einheitlichen Methode berechnet. In dieser ersten Arbeit wird die Berechnung der Dielektrizitätskonstanten und der Leitfähigkeiten für Elektrizität und Wärme der Mischkörper aus isotropen Bestandteilen behandelt. Die Genauigkeit der älteren Formeln wird untersucht und die bis jetzt unbekannten Konstanten dieser Formeln werden berechnet. Sodann wird die Theorie geprüft an Messungen der Leitfähigkeit bei heterogenen Metallegierungen und an den DK. von gepreßten Pulvern und Emulsionen; die verschiedenen Formeln werden bestätigt. Bei dieser Anwendung werden einige Widersprüche zwischen früheren Untersuchungen aufgehoben und es wird versucht, einige ungenau bekannte DK. genauer zu bestimmen.},
year = {1935}
}

@article{larsen2016robust,
  title={Robust structural identification via polyhedral template matching},
  author={Larsen, Peter Mahler and Schmidt, S{\o}ren and Schi{\o}tz, Jakob},
  journal={Modelling and Simulation in Materials Science and Engineering},
  volume={24},
  number={5},
  pages={055007},
  year={2016},
  publisher={IOP Publishing}
}


@Article{mirigliano2020b,
author={Mirigliano, M.
and Radice, S.
and Falqui, A.
and Casu, A.
and Cavaliere, F.
and Milani, P.},
title={Anomalous electrical conduction and negative temperature coefficient of resistance in nanostructured gold resistive switching films},
journal={Scientific Reports},
year={2020},
month={Nov},
day={12},
volume={10},
number={1},
pages={19613},
abstract={We report the observation of non-metallic electrical conduction, resistive switching, and a negative temperature coefficient of resistance in nanostructured gold films above the electrical percolation and in strong-coupling regime, from room down to cryogenic temperatures (24 K). Nanostructured continuous gold films are assembled by supersonic cluster beam deposition of Au aggregates formed in the gas phase. The structure of the cluster-assembled films is characterized by an extremely high density of randomly oriented crystalline nanodomains, separated by grain boundaries and with a large number of lattice defects. Our data indicates that space charge limited conduction and Coulomb blockade are at the origin of the anomalous electrical behavior. The high density of extended defects and grain boundaries causes the localization of conduction electrons over the entire investigated temperature range.},
issn={2045-2322},
doi={10.1038/s41598-020-76632-y},
url={https://doi.org/10.1038/s41598-020-76632-y}
}


@article{mirigliano2021a,
author = {Matteo Mirigliano and Paolo Milani},
title = {Electrical conduction in nanogranular cluster-assembled metallic films},
journal = {Advances in Physics: X},
volume = {6},
number = {1},
pages = {1908847},
year  = {2021},
publisher = {Taylor & Francis},
doi = {10.1080/23746149.2021.1908847},

URL = { 
        https://doi.org/10.1080/23746149.2021.1908847
    
},
eprint = { 
        https://doi.org/10.1080/23746149.2021.1908847
    
}

}


@book{choy2015,
  title={Effective Medium Theory: Principles and Applications},
  author={Choy, T.C.},
  isbn={9780191015182},
  series={International Series of Monographs on Physics},
  url={https://books.google.it/books?id=sHUgCwAAQBAJ},
  year={2015},
  publisher={OUP Oxford}
}
@article{henriquez2013,
title = "Electron scattering at surfaces and grain boundaries in thin Au films",
journal = "Applied Surface Science",
volume = "273",
pages = "315 - 323",
year = "2013",
issn = "0169-4332",
doi = "https://doi.org/10.1016/j.apsusc.2013.02.037",
url = "http://www.sciencedirect.com/science/article/pii/S0169433213003450",
author = "Ricardo Henriquez and Marcos Flores and Luis Moraga and German Kremer and Claudio González-Fuentes and Raul C. Munoz",
keywords = "Resistivity, Electron-surface scattering, Electron-grain boundary scattering",
abstract = ""
}

@article{munoz2017size,
  title={Size effects and charge transport in metals: Quantum theory of the resistivity of nanometric metallic structures arising from electron scattering by grain boundaries and by rough surfaces},
  author={Munoz, Raul C and Arenas, Claudio},
  journal={Applied Physics Reviews},
  volume={4},
  number={1},
  pages={011102},
  year={2017},
  publisher={AIP Publishing LLC}
}


@article{fuchs1938, title={The conductivity of thin metallic films according to the electron theory of metals}, volume={34}, DOI={10.1017/S0305004100019952}, number={1}, journal={Mathematical Proceedings of the Cambridge Philosophical Society}, publisher={Cambridge University Press}, author={Fuchs, K.}, year={1938}, pages={100–108}}

@article{sondheimer1952,
author = { E.H.   Sondheimer },
title = {The mean free path of electrons in metals},
journal = {Advances in Physics},
volume = {1},
number = {1},
pages = {1-42},
year  = {1952},
publisher = {Taylor \& Francis},
doi = {10.1080/00018735200101151},

URL = {
        https://doi.org/10.1080/00018735200101151

}
}
@article{borziak1976,
title = "Electrical conductivity in structurally inhomogeneous discontinuous metal films",
journal = "Thin Solid Films",
volume = "36",
number = "1",
pages = "21 - 24",
year = "1976",
issn = "0040-6090",
doi = "https://doi.org/10.1016/0040-6090(76)90389-8",
url = "http://www.sciencedirect.com/science/article/pii/0040609076903898",
author = "P Borziak and V Dyukov and A Kostenko and Yu Kulyupin and S Nepijko"
}
@article{sattar2013,
  title = {Quantized Conductance and Switching in Percolating Nanoparticle Films},
  author = {Sattar, Abdul and Fostner, Shawn and Brown, Simon A.},
  journal = {Phys. Rev. Lett.},
  volume = {111},
  issue = {13},
  pages = {136808},
  numpages = {5},
  year = {2013},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.111.136808},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.111.136808}
}

@article{mayadas1970,
  title = {Electrical-Resistivity Model for Polycrystalline Films: the Case of Arbitrary Reflection at External Surfaces},
  author = {Mayadas, A. F. and Shatzkes, M.},
  journal = {Phys. Rev. B},
  volume = {1},
  issue = {4},
  pages = {1382--1389},
  numpages = {0},
  year = {1970},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.1.1382},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.1.1382}
}
@article{tarantino2020,
  title = {Modeling resistive switching in nanogranular metal films},
  author = {Tarantino, Walter and Colombo, Luciano},
  journal = {Phys. Rev. Research},
  volume = {2},
  issue = {4},
  pages = {043389},
  numpages = {9},
  year = {2020},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.2.043389},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.2.043389}
}

@article{mirigliano2020,
	doi = {10.1088/1361-6528/ab76ec},
	url = {https://doi.org/10.1088%2F1361-6528%2Fab76ec},
	year = 2020,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {31},
	number = {23},
	pages = {234001},
	author = {M Mirigliano and D Decastri and A Pullia and D Dellasega and A Casu and A Falqui and P Milani},
	title = {Complex electrical spiking activity in resistive switching nanostructured Au two-terminal devices},
	journal = {Nanotechnology},
	abstract = {Networks of nanoscale objects are the subject of increasing interest as resistive switching systems for the fabrication of neuromorphic computing architectures. Nanostructured films of bare gold clusters produced in gas phase with thickness well beyond the electrical percolation threshold, show a non-ohmic electrical behavior and resistive switching, resulting in groups of current spikes with irregular temporal organization. Here we report the systematic characterization of the temporal correlations between single spikes and spiking rate power spectrum of nanostructured Au two-terminal devices consisting of a cluster-assembled film deposited between two planar electrodes. By varying the nanostructured film thickness we fabricated two different classes of devices with high and low initial resistance respectively. We show that the switching dynamics can be described by a power law distribution in low resistance devices whereas a bi-exponential behavior is observed in the high resistance ones. The measured resistance of cluster-assembled films shows a  scaling behavior in the range of analyzed frequencies. Our results suggest the possibility of using cluster-assembled Au films as components for neuromorphic systems where a certain degree of stochasticity is required.}
}
@article{falcon2017,
  title = {Pressure dependence of the electrical transport in granular materials},
  author = {Creyssels, M. and Laroche, C. and Falcon, E. and Castaing, B.},
  journal = {Eur. Phys. J. E},
  volume = {40},
  issue = {56},
  pages = {},
  numpages = {0},
  year = {2017},
  month = {May},
  publisher = {Springer},
  doi = {10.1140/epje/i2017-11543-3},
  url = {https://doi.org/10.1140/epje/i2017-11543-3}
}


@article{kirkpatrick1973,
  title = {Percolation and Conduction},
  author = {Kirkpatrick, Scott},
  journal = {Rev. Mod. Phys.},
  volume = {45},
  issue = {4},
  pages = {574--588},
  numpages = {0},
  year = {1973},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.45.574},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.45.574}
}

@incollection{bergman1992,
title = "Physical Properties of Macroscopically Inhomogeneous Media",
editor = "HENRY EHRENREICH and DAVID TURNBULL",
series = "Solid State Physics",
publisher = "Academic Press",
volume = "46",
pages = "147 - 269",
year = "1992",
issn = "0081-1947",
doi = "https://doi.org/10.1016/S0081-1947(08)60398-7",
url = "http://www.sciencedirect.com/science/article/pii/S0081194708603987",
author = "David J. Bergman and David Stroud",
abstract = "Publisher Summary
This chapter discusses several composites or granular or porous materials that display inhomogeneity on a macroscopic scale. In such materials, there are small, yet much larger than atomic, regions exhibiting macroscopic homogeneity. Different regions may display quite different properties. The chapter discusses the dc and ac electrical properties of composite media including the basic theory and results for dc electrical properties. It also presents a discussion of the effective-medium approximation, electrostatic resonances, exact bounds, and analytical properties and describes a number of static physical properties of composites. These properties include electrical conductivity and dielectric behavior near a percolation threshold, magnetotransport, thermoelectricity, superconductivity, and duality in two-dimensional composites. Finally, the chapter discusses the nonlinear properties and flicker noise in composites."
}



@Book{tipler1999,
title = {Physics for scientists and engineers},
author = { Tipler, Paul A. (Paul Allen) },
publisher = { New York : W.H. Freeman },
year = { 1999 },
type = { Book; Book/Illustrated },
edition = { 4th ed },
isbn = { 1572596732 (pbk.) },
subjects = { Physics },
note = { Includes bibliographical references and index },
catalogue-url = { https://trove.nla.gov.au/work/9589101 }
}
@Book{giancoli2005,
title = { Physics : principles with applications },
author = { Giancoli, Douglas C },
url = { http://www.ulb.tu-darmstadt.de/tocs/133387143.pdf },
publisher = { Upper Saddle River, N.J. : Pearson Education },
year = { 2005 },
type = { Book; Book/Illustrated },
edition = { 6th International ed },
isbn = { 013191183X (International ed. : alk. paper) },
subjects = { Physik; Physics - Year 12; Physics; Physics - Year 11 },
note = { Includes index },
contents = { V1. Chapters 1-15 -- V2. Chapters 16-33. -- International edition: Chapters 1 - 33 },
catalogue-url = { https://trove.nla.gov.au/work/5654727 }
}

@article{ederth2000,
author = {Ederth,J.  and Kish,L. B.  and Olsson,E.  and Granqvist,C. G. },
title = {Temperature dependent electrical resistivity in nanocrystalline gold films made by advanced gas deposition},
journal = {Journal of Applied Physics},
volume = {88},
number = {11},
pages = {6578-6582},
year = {2000},
doi = {10.1063/1.1322384},

URL = { 
        https://doi.org/10.1063/1.1322384
    
},

}


@book{serway1998,
  title={Principles of Physics},
  author={Serway, R.A. and Gordon, J.R.},
  number={v. 2},
  isbn={9780030246289},
  series={Principles of Physics},
  url={https://books.google.it/books?id=9FG6skFea48C},
  year={1998},
  publisher={Saunders College Pub.}
}

@article{grimaldi2014,
  title = {Theory of percolation and tunneling regimes in nanogranular metal films},
  author = {Grimaldi, Claudio},
  journal = {Phys. Rev. B},
  volume = {89},
  issue = {21},
  pages = {214201},
  numpages = {11},
  year = {2014},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.89.214201},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.89.214201}
}


@misc{invertastic,
    author = "Alan Gray",
    title = "Invertastic: Large-scale Dense Matrix Inversion",
    year = "2016",
    url  = "https://www.archer.ac.uk/documentation/white-papers/invertastic/invertasticGray.pdf"
}

@book{stewart2009,
  title={Probability, Markov Chains, Queues, and Simulation: The Mathematical Basis of Performance Modeling},
  author={Stewart, W.J.},
  isbn={9781400832811},
  url={https://books.google.it/books?id=ZfRyBS1WbAQC},
  year={2009},
  publisher={Princeton University Press}
}
@article{lee2020,
author={Lee, Seung Hwan
and Zhu, Xiaojian
and Lu, Wei D.},
title={Nanoscale resistive switching devices for memory and computing applications},
journal={Nano Research},
year={2020},
month={Jan},
day={17},
abstract={With the slowing down of the Moore's law and fundamental limitations due to the von-Neumann bottleneck, continued improvements in computing hardware performance become increasingly more challenging. Resistive switching (RS) devices are being extensively studied as promising candidates for next generation memory and computing applications due to their fast switching speed, excellent endurance and retention, and scaling and three-dimensional (3D) stacking capability. In particular, RS devices offer the potential to natively emulate the functions and structures of synapses and neurons, allowing them to efficiently implement neural networks (NNs) and other in-memory computing systems for data intensive applications such as machine learning tasks. In this review, we will examine the mechanisms of RS effects and discuss recent progresses in the application of RS devices for memory, deep learning accelerator, and more faithful brain-inspired computing tasks. Challenges and possible solutions at the device, algorithm, and system levels will also be discussed.},
issn={1998-0000},
doi={10.1007/s12274-020-2616-0},
url={https://doi.org/10.1007/s12274-020-2616-0}
}
@article{chen2018,
title = "Neuromorphic computing's yesterday, today, and tomorrow – an evolutional view",
journal = "Integration",
volume = "61",
pages = "49 - 61",
year = "2018",
issn = "0167-9260",
doi = "https://doi.org/10.1016/j.vlsi.2017.11.001",
url = "http://www.sciencedirect.com/science/article/pii/S0167926017304674",
author = "Yiran Chen and Hai (Helen) Li and Chunpeng Wu and Chang Song and Sicheng Li and Chuhan Min and Hsin-Pai Cheng and Wei Wen and Xiaoxiao Liu",
keywords = "Neuromorphic computing, Brain-inspired computing, Machine learning, Deep learning",
abstract = "Neuromorphic computing was originally referred to as the hardware that mimics neuro-biological architectures to implement models of neural systems. The concept was then extended to the computing systems that can run bio-inspired computing models, e.g., neural networks and deep learning networks. In recent years, the rapid growth of cognitive applications and the limited processing capability of conventional von Neumann architecture on these applications motivated worldwide research on neuromorphic computing systems. In this paper, we review the evolution of neuromorphic computing technique in both computing model and hardware implementation from a historical perspective. Various implementation methods and practices are also discussed. Finally, we present some emerging technologies that may potentially change the landscape of neuromorphic computing in the future, e.g., new devices and interdisciplinary computing architectures."
}






@article{gall2016,
author = {Gall,Daniel },
title = {Electron mean free path in elemental metals},
journal = {Journal of Applied Physics},
volume = {119},
number = {8},
pages = {085101},
year = {2016},
doi = {10.1063/1.4942216},
URL = {https://doi.org/10.1063/1.4942216}
}

@article{lee2015,
author = {Lee,Jae Sung  and Lee,Shinbuhm  and Noh,Tae Won },
title = {Resistive switching phenomena: A review of statistical physics approaches},
journal = {Applied Physics Reviews},
volume = {2},
number = {3},
pages = {031303},
year = {2015},
doi = {10.1063/1.4929512},
URL = { 
        https://doi.org/10.1063/1.4929512
},
eprint = { 
        https://doi.org/10.1063/1.4929512
    }
}
@article{hwang2019,
author = {Hwang, Bohee and Lee, Jang-Sik},
title = {Recent Advances in Memory Devices with Hybrid Materials},
journal = {Advanced Electronic Materials},
volume = {5},
number = {1},
pages = {1800519},
keywords = {composite layers, hybrid materials, memory devices, organic–inorganic hybrid perovskites, resistive switching memory},
doi = {10.1002/aelm.201800519},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/aelm.201800519},
eprint = {},
abstract = {Abstract Increasing demands for information-storage capacity and for miniaturization of memory cells have driven exploration of new-generation data storage devices, because the conventional Si-based memory technology is approaching its fundamental physical limits. Hybrid materials and novel device structure may lead to a paradigm shift toward memory devices that have high density, multifunctionality, and low power consumption. Here, the structure and operation mechanism of resistive switching memory devices are described, then recent advances in hybrid materials (e.g., graphene-based polymer composites, organic–inorganic hybrid perovskite materials) for fabrication of these devices are summarized. How to increase the ON/OFF ratio and the density of memories, and to decrease programming voltage by selecting appropriate active materials, and engineering the active layers, are also demonstrated. Finally, the current challenges and future directions in memory devices based on hybrid materials are summarized.},
year = {2019}
}
@article{stroud1998,
title = "The effective medium approximations: Some recent developments",
journal = "Superlattices and Microstructures",
volume = "23",
number = "3",
pages = "567 - 573",
year = "1998",
issn = "0749-6036",
doi = "https://doi.org/10.1006/spmi.1997.0524",
url = "http://www.sciencedirect.com/science/article/pii/S0749603697905243",
author = "D. Stroud",
keywords = "composite, effective medium, percolation, noise",
abstract = "We provide a brief and highly selective review of the Landauer– Bruggeman effective-medium approximation as applied to random composite media. We first discuss this approximation as applied to linear composites, i.e., to those materials in which there is a linear relation between a curl-free electric field and a divergence-free current density. We then describe extensions of this approach to random composites with cubic nonlinearities in addition to a dominant linear term, and to composites in which the components have a fluctuating conductivity (‘conductivity noise’). Finally, we mention one novel application: to conductivity noise in a random composite of normal metal (N) and perfect conductor (S). It is shown that the extension of the EMA leads to a prediction of a frequency range in which the conductivity noise has a 1/ω frequency dependence, even if the noise in the individual components is frequency independent."
}

@article{fostner2014,
  title = {Continuum percolation with tunneling},
  author = {Fostner, Shawn and Brown, Richard and Carr, James and Brown, Simon A.},
  journal = {Phys. Rev. B},
  volume = {89},
  issue = {7},
  pages = {075402},
  numpages = {4},
  year = {2014},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.89.075402},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.89.075402}
}

@Article{Diaz-Alvarez_2019,
author={Diaz-Alvarez, Adrian
and Higuchi, Rintaro
and Sanz-Leon, Paula
and Marcus, Ido
and Shingaya, Yoshitaka
and Stieg, Adam Z.
and Gimzewski, James K.
and Kuncic, Zdenka
and Nakayama, Tomonobu},
title={Emergent dynamics of neuromorphic nanowire networks},
journal={Scientific Reports},
year={2019},
month={Oct},
day={17},
volume={9},
number={1},
pages={14920},
abstract={Neuromorphic networks are formed by random self-assembly of silver nanowires. Silver nanowires are coated with a polymer layer after synthesis in which junctions between two nanowires act as resistive switches, often compared with neurosynapses. We analyze the role of single junction switching in the dynamical properties of the neuromorphic network. Network transitions to a high-conductance state under the application of a voltage bias higher than a threshold value. The stability and permanence of this state is studied by shifting the voltage bias in order to activate or deactivate the network. A model of the electrical network with atomic switches reproduces the relation between individual nanowire junctions switching events with current pathway formation or destruction. This relation is further manifested in changes in 1/f power-law scaling of the spectral distribution of current. The current fluctuations involved in this scaling shift are considered to arise from an essential equilibrium between formation, stochastic-mediated breakdown of individual nanowire-nanowire junctions and the onset of different current pathways that optimize power dissipation. This emergent dynamics shown by polymer-coated Ag nanowire networks places this system in the class of optimal transport networks, from which new fundamental parallels with neural dynamics and natural computing problem-solving can be drawn.},
issn={2045-2322},
doi={10.1038/s41598-019-51330-6},
url={https://doi.org/10.1038/s41598-019-51330-6}
}


@Article{yang2013,
author ="Yang, Yuchao and Lu, Wei",
title  ="Nanoscale resistive switching devices: mechanisms and modeling",
journal  ="Nanoscale",
year  ="2013",
volume  ="5",
issue  ="21",
pages  ="10076-10092",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C3NR03472K",
url  ="http://dx.doi.org/10.1039/C3NR03472K",
abstract  ="Resistive switching devices (also termed memristive devices or memristors) are two-terminal nonlinear dynamic electronic devices that can have broad applications in the fields of nonvolatile memory{,} reconfigurable logic{,} analog circuits{,} and neuromorphic computing. Current rapid advances in memristive devices in turn demand better understanding of the switching mechanism and the development of physics-based as well as simplified device models to guide future device designs and circuit-level applications. In this article{,} we review the physical processes behind resistive switching (memristive) phenomena and discuss the experimental and modeling efforts to explain these effects. In this article three categories of devices{,} in which the resistive switching effects are driven by cation migration{,} anion migration{,} and electronic effects{,} will be discussed. The fundamental driving forces and the stochastic nature of resistive switching will also be discussed."}


@article{sillin2013,
	doi = {10.1088/0957-4484/24/38/384004},
	url = {https://doi.org/10.1088%2F0957-4484%2F24%2F38%2F384004},
	year = 2013,
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {24},
	number = {38},
	pages = {384004},
	author = {Henry O Sillin and Renato Aguilera and Hsien-Hang Shieh and Audrius V Avizienis and Masakazu Aono and Adam Z Stieg and James K Gimzewski},
	title = {A theoretical and experimental study of neuromorphic atomic switch networks for reservoir computing},
	journal = {Nanotechnology},
	abstract = {Atomic switch networks (ASNs) have been shown to generate network level dynamics that resemble those observed in biological neural networks. To facilitate understanding and control of these behaviors, we developed a numerical model based on the synapse-like properties of individual atomic switches and the random nature of the network wiring. We validated the model against various experimental results highlighting the possibility to functionalize the network plasticity and the differences between an atomic switch in isolation and its behaviors in a network. The effects of changing connectivity density on the nonlinear dynamics were examined as characterized by higher harmonic generation in response to AC inputs. To demonstrate their utility for computation, we subjected the simulated network to training within the framework of reservoir computing and showed initial evidence of the ASN acting as a reservoir which may be optimized for specific tasks by adjusting the input gain. The work presented represents steps in a unified approach to experimentation and theory of complex systems to make ASNs a uniquely scalable platform for neuromorphic computing.}
}






@article{Pike_2020,
author = {Pike, Matthew D. and Bose, Saurabh K. and Mallinson, Joshua B. and Acharya, Susant K. and Shirai, Shota and Galli, Edoardo and Weddell, Stephen J. and Bones, Philip J. and Arnold, Matthew D. and Brown, Simon A.},
title = {Atomic Scale Dynamics Drive Brain-like Avalanches in Percolating Nanostructured Networks},
journal = {Nano Letters},
volume = {20},
number = {5},
pages = {3935-3942},
year = {2020},
doi = {10.1021/acs.nanolett.0c01096},
    note ={PMID: 32347733},

URL = { 
        https://doi.org/10.1021/acs.nanolett.0c01096
    
},

}



@article{Milano_2020,
author = {Milano, Gianluca and Pedretti, Giacomo and Fretto, Matteo and Boarino, Luca and Benfenati, Fabio and Ielmini, Daniele and Valov, Ilia and Ricciardi, Carlo},
title = {Brain-Inspired Structural Plasticity through Reweighting and Rewiring in Multi-Terminal Self-Organizing Memristive Nanowire Networks},
journal = {Advanced Intelligent Systems},
volume = {2},
number = {8},
pages = {2000096},
keywords = {heterosynaptic plasticity, memristive systems, nanoarchitectures, nanowire networks, neuromorphic systems},
doi = {https://doi.org/10.1002/aisy.202000096},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/aisy.202000096},
abstract = {Acting as artificial synapses, two-terminal memristive devices are considered fundamental building blocks for the realization of artificial neural networks. Current memristive crossbar architectures demonstrate the implementation of neuromorphic computing paradigms, although they are unable to emulate typical features of biological neural networks such as high connectivity, adaptability through reconnection and rewiring, and long-range spatio-temporal correlation. Herein, self-organizing memristive random nanowire (NW) networks with functional connectivity able to display homo- and heterosynaptic plasticity is reported thanks to the mutual electrochemical interaction among memristive NWs and NW junctions. In particular, it is shown that rewiring and reweighting effects observed in single NWs and single NW junctions, respectively, are responsible for structural plasticity of the network under electrical stimulation. Such biologically inspired systems allow a low-cost realization of neural networks that can learn and adapt when subjected to multiple external stimuli, emulating the experience-dependent synaptic plasticity that shape the connectivity and functionalities of the nervous system that can be exploited for hardware implementation of unconventional computing paradigms.},
year = {2020}
}



@Article{Manning_2018,
author={Manning, Hugh G.
and Niosi, Fabio
and da Rocha, Claudia Gomes
and Bellew, Allen T.
and O'Callaghan, Colin
and Biswas, Subhajit
and Flowers, Patrick F.
and Wiley, Benjamin J.
and Holmes, Justin D.
and Ferreira, Mauro S.
and Boland, John J.},
title={Emergence of winner-takes-all connectivity paths in random nanowire networks},
journal={Nature Communications},
year={2018},
month={Aug},
day={13},
volume={9},
number={1},
pages={3219},
abstract={Nanowire networks are promising memristive architectures for neuromorphic applications due to their connectivity and neurosynaptic-like behaviours. Here, we demonstrate a self-similar scaling of the conductance of networks and the junctions that comprise them. We show this behavior is an emergent property of any junction-dominated network. A particular class of junctions naturally leads to the emergence of conductance plateaus and a ``winner-takes-all'' conducting path that spans the entire network, and which we show corresponds to the lowest-energy connectivity path. The memory stored in the conductance state is distributed across the network but encoded in specific connectivity pathways, similar to that found in biological systems. These results are expected to have important implications for development of neuromorphic devices based on reservoir computing.},
issn={2041-1723},
doi={10.1038/s41467-018-05517-6},
url={https://doi.org/10.1038/s41467-018-05517-6}
}


@article {Mallinson_2019,
	author = {Mallinson, J. B. and Shirai, S. and Acharya, S. K. and Bose, S. K. and Galli, E. and Brown, S. A.},
	title = {Avalanches and criticality in self-organized nanoscale networks},
	volume = {5},
	number = {11},
	elocation-id = {eaaw8438},
	year = {2019},
	doi = {10.1126/sciadv.aaw8438},
	publisher = {American Association for the Advancement of Science},
	abstract = {Current efforts to achieve neuromorphic computation are focused on highly organized architectures, such as integrated circuits and regular arrays of memristors, which lack the complex interconnectivity of the brain and so are unable to exhibit brain-like dynamics. New architectures are required, both to emulate the complexity of the brain and to achieve critical dynamics and consequent maximal computational performance. We show here that electrical signals from self-organized networks of nanoparticles exhibit brain-like spatiotemporal correlations and criticality when fabricated at a percolating phase transition. Specifically, the sizes and durations of avalanches of switching events are power law distributed, and the power law exponents satisfy rigorous criteria for criticality. These signals are therefore qualitatively and quantitatively similar to those measured in the cortex. Our self-organized networks provide a low-cost platform for computational approaches that rely on spatiotemporal correlations, such as reservoir computing, and are an important step toward creating neuromorphic device architectures.},
	URL = {https://advances.sciencemag.org/content/5/11/eaaw8438},
	journal = {Science Advances}
}

@ARTICLE{Loeffler_2020,
  
AUTHOR={Loeffler, Alon and Zhu, Ruomin and Hochstetter, Joel and Li, Mike and Fu, Kaiwei and Diaz-Alvarez, Adrian and Nakayama, Tomonobu and Shine, James M. and Kuncic, Zdenka},   
	 
TITLE={Topological Properties of Neuromorphic Nanowire Networks},      
	
JOURNAL={Frontiers in Neuroscience},      
	
VOLUME={14},      

PAGES={184},     
	
YEAR={2020},      
	  
URL={https://www.frontiersin.org/article/10.3389/fnins.2020.00184},       
	
DOI={10.3389/fnins.2020.00184},      
	
ISSN={1662-453X},   
   
ABSTRACT={Graph theory has been extensively applied to the topological mapping of complex networks, ranging from social networks to biological systems. Graph theory has increasingly been applied to neuroscience as a method to explore the fundamental structural and functional properties of human neural networks. Here, we apply graph theory to a model of a novel neuromorphic system constructed from self-assembled nanowires, whose structure and function may mimic that of human neural networks. Simulations of neuromorphic nanowire networks allow us to directly examine their topology at the individual nanowire–node scale. This type of investigation is currently extremely difficult experimentally. We then apply network cartographic approaches to compare neuromorphic nanowire networks with: random networks (including an untrained artificial neural network); grid-like networks and the structural network of C. elegans. Our results demonstrate that neuromorphic nanowire networks exhibit a small–world architecture similar to the biological system of C. elegans, and significantly different from random and grid-like networks. Furthermore, neuromorphic nanowire networks appear more segregated and modular than random, grid-like and simple biological networks and more clustered than artificial neural networks. Given the inextricable link between structure and function in neural networks, these results may have important implications for mimicking cognitive functions in neuromorphic nanowire networks.}
}
@article{fostner2015,
  title = {Neuromorphic behavior in percolating nanoparticle films},
  author = {Fostner, Shawn and Brown, Simon A.},
  journal = {Phys. Rev. E},
  volume = {92},
  issue = {5},
  pages = {052134},
  numpages = {11},
  year = {2015},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.92.052134},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.92.052134}
}

@article{beloborodov2007granular,
  title={Granular electronic systems},
  author={Beloborodov, IS and Lopatin, AV and Vinokur, VM and Efetov, KB},
  journal={Reviews of Modern Physics},
  volume={79},
  number={2},
  pages={469},
  year={2007},
  publisher={APS}
}

@incollection{morris2008,
  author       = {Morris, James E.}, 
  title        = {Nanoparticle Properties},
  booktitle    = {Nanopackaging},
  publisher    = {Springer US},
  year         = 2008,
  editor       = {Morris, James E.},
  volume       = {},
  series       = {},
  chapter      = 5,
  pages        = {93-107},
  address      = {},
  edition      = 1,
  month        = {},
  note         = {}
}


@Article{minnai2017,
author={Minnai, Chlo{\'e}
and Bellacicca, Andrea
and Brown, Simon A.
and Milani, Paolo},
title={Facile fabrication of complex networks of memristive devices},
journal={Scientific Reports},
year={2017},
month={Aug},
day={11},
volume={7},
number={1},
pages={7955},
abstract={We describe the memristive properties of cluster-assembled gold films. We show that resistive switching is observed in pure metallic nanostructured films at room temperature and atmospheric pressure, in response to applied voltage inputs. In particular, we observe resistance changes up to 400{\%} and archetypal switching events that have remarkable symmetry with the applied voltage. We associated this symmetry with `potentiation' and `anti-potentiation' processes involving the activation of synapses and of pathways comprising multiple synapses. The stability and reproducibility of the resistance switching, which lasted over many hours, make these devices ideal test-beds for exploration of the basic mechanisms of the switching processes, and allow convenient fabrication of devices that may have neuromorphic properties.},
issn={2045-2322},
doi={10.1038/s41598-017-08244-y},
url={https://doi.org/10.1038/s41598-017-08244-y}
}



@book{stauffer1994,
  title={Introduction To Percolation Theory},
  author={Stauffer, D. and Aharony, A.},
  isbn={9781420074796},
  url={https://books.google.it/books?id=v66plleij5QC},
  year={1994},
  publisher={Taylor \& Francis}
}
@book{sahimi1994,
  title={Applications Of Percolation Theory},
  author={Sahimi, M.},
  isbn={9780748400768},
  lccn={lc93033032},
  url={https://books.google.it/books?id=lTO01mZsVhsC},
  year={1994},
  publisher={Taylor \& Francis}
}

@article{luck1991,
  title = {Conductivity of random resistor networks: An investigation of the accuracy of the effective-medium approximation},
  author = {Luck, J. M.},
  journal = {Phys. Rev. B},
  volume = {43},
  issue = {5},
  pages = {3933--3944},
  numpages = {0},
  year = {1991},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.43.3933},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.43.3933}
}
@article{vionnetmenot2005,
  title = {Tunneling-percolation origin of nonuniversality: Theory and experiments},
  author = {Vionnet-Menot, Sonia and Grimaldi, Claudio and Maeder, Thomas and Str\"assler, Sigfrid and Ryser, Peter},
  journal = {Phys. Rev. B},
  volume = {71},
  issue = {6},
  pages = {064201},
  numpages = {12},
  year = {2005},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.71.064201},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.71.064201}
}
@article{grimaldi2006,
  title = {Tunneling and Nonuniversality in Continuum Percolation Systems},
  author = {Grimaldi, C. and Balberg, I.},
  journal = {Phys. Rev. Lett.},
  volume = {96},
  issue = {6},
  pages = {066602},
  numpages = {4},
  year = {2006},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.96.066602},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.96.066602}
}











%%%%%%%%%%%%%%%%%%%%%%  END GRANECO 2019  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BOOK %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@book{berestetskii,
      author         = "Akhiezer, A. I. and Berestetskii, V. B.",
      title          = "{Quantum electrodynamics}",
      year           = "1965",
      reportNumber   = "AEC-TR-2876",
      SLACcitation   = "%%CITATION = AEC-TR-2876;%%"
}
@book{strange1998,
  title={Relativistic Quantum Mechanics: With Applications in Condensed Matter and Atomic Physics},
  author={Strange, P.},
  isbn={9780521565837},
  lccn={97018019},
  url={http://books.google.ch/books?id=sdVrBM2w0OwC},
  year={1998},
  publisher={Cambridge University Press}
}
@book{itz,
  title={Quantum Field Theory},
  author={Itzykson, C.G. and Zuber, J.B.},
  isbn={9780486445687},
  lccn={2005053026},
  series={Dover Books on Physics},
  url={http://books.google.ch/books?id=baqXmAEACAAJ},
  year={2005},
  publisher={Dover Publications, Incorporated}
}
@book{engeldreizler2011,
  title={Density Functional Theory: An Advanced Course},
  author={Engel, E. and Dreizler, R.M.},
  isbn={9783642140907},
  series={Texts and Monographs in Physics},
  url={http://books.google.ch/books?id=R2\_RBzVu3TUC},
  year={2011},
  publisher={Springer Berlin Heidelberg}
}
@book{ullrich2012,
  title={Time-Dependent Density-Functional Theory: Concepts and Applications},
  author={Ullrich, C.A.},
  isbn={9780199563029},
  lccn={2012382303},
  series={Oxford Graduate Texts},
  url={http://books.google.ch/books?id=j\_4nodMFCa4C},
  year={2012},
  publisher={OUP Oxford}
}
@book{griffiths2008,
  title={Introduction to Elementary Particles},
  author={Griffiths, D.},
  isbn={9783527406012},
  series={Physics Textbook},
  url={http://books.google.ch/books?id=w9Dz56myXm8C},
  year={2008},
  publisher={Wiley}
}
@book{ryder,
  title={Quantum Field Theory},
  author={Ryder, L.H.},
  isbn={9780521478144},
  lccn={95031119},
  url={http://books.google.ch/books?id=nnuW\_kVJ500C},
  year={1996},
  publisher={Cambridge University Press}
}
@book{peskin,
  title={An Introduction To Quantum Field Theory},
  author={Peskin, M.E. and Schroeder, D.V.},
  isbn={9780813345437},
  series={Frontiers in physics},
  url={http://books.google.ch/books?id=EVeNNcslvX0C},
  year={1995},
  publisher={Westview Press}
}
@book{umezawa,
  title={Thermo field dynamics and condensed states},
  author={Umezawa, H. and Matsumoto, H. and Tachiki, M.},
  isbn={9780444863614},
  lccn={lc81022491},
  url={http://books.google.co.uk/books?id=Ra7vAAAAMAAJ},
  year={1982},
  publisher={North-Holland Pub. Co.}
}
@book{dreizlergross1990,
  title={Density Functional Theory: An Approach to the Quantum Many- Body Problem},
  author={Dreizler, R.M. and Gross, E.K.U.},
  isbn={9780387519937},
  lccn={90009623},
  url={http://books.google.ch/books?id=QAB-QgAACAAJ},
  year={1990},
  publisher={Springer-Verlag}
}
@book{joubert2002,
  title={Density Functionals: Theory and Applications: Proceedings of the Tenth Chris Engelbrecht Summer School in Theoretical Physics Held at Meerensee, near Cape Town, South Africa, 19-29 January 1997},
  author={Joubert, D.},
  isbn={9783540639374},
  lccn={97051526},
  series={Lecture Notes in Physics},
  url={http://books.google.ch/books?id=GFTXRYmQdiQC},
  year={2002},
  publisher={Springer}
}
@book{marques2003,
  title={A Primer in Density Functional Theory},
  author={Fiolhais, C. and Nogueira, F. and Marques, M.A.L.},
  isbn={9783540030836},
  lccn={03050612},
  series={Lecture Notes in Physics},
  url={http://books.google.ch/books?id=mX793GABep8C},
  year={2003},
  publisher={Springer}
}
@book{bacry1988,
title={Localizability and Space in Quantum Physics},
author={Bacry, Henri},
isbn={978-3-540-50052-0},
year={1988},
volume={308},
series={Lecture Notes in Physics},
doi={10.1007/BFb0019324},
url={http://dx.doi.org/10.1007/BFb0019324},
publisher={Springer Berlin Heidelberg},
}
@book{scully,
  title={Quantum Optics},
  author={Scully, M.O. and Zubairy, S.},
  isbn={9780521435956},
  lccn={94042949},
  url={http://books.google.de/books?id=20ISsQCKKmQC},
  year={1997},
  publisher={Cambridge University Press}
}
@book{thaller,
  title={The Dirac equation},
  author={Thaller, B.},
  isbn={9783540548836},
  lccn={92012288},
  series={Texts and monographs in physics},
  url={http://books.google.fr/books?id=X7XvAAAAMAAJ},
  year={1992},
  publisher={Springer-Verlag}
}
@book{friedrichs,
  title={Mathematical aspects of the quantum theory of fields},
  author={Friedrichs, K.O.},
  lccn={lc53007156},
  url={http://books.google.de/books?id=B-o-AAAAIAAJ},
  year={1953},
  publisher={Interscience Publishers}
}
@book{schweber,
  title={An Introduction to Relativistic Quantum Field Theory},
  author={Schweber, S.S.},
  isbn={9780486139609},
  url={http://books.google.co.uk/books?id=v1owGsfiJcoC},
  year={2011},
  publisher={Dover Publications}
}
@book{milonni,
  title={The quantum vacuum: an introduction to quantum electrodynamics},
  author={Milonni, P.W.},
  isbn={9780124980808},
  lccn={93029780},
  url={http://books.google.de/books?id=P83vAAAAMAAJ},
  year={1994},
  publisher={Academic Press}
}
@book{birrell,
  title={Quantum Fields in Curved Space},
  author={Birrell, N.D. and Davies, P.C.W.},
  isbn={9780521278584},
  lccn={86707777},
  series={Cambridge Monographs on Mathematical Physics},
  url={http://books.google.de/books?id=SEnaUnrqzrUC},
  year={1984},
  publisher={Cambridge University Press}
}
@book{wald1994,
  title={Quantum Field Theory in Curved Spacetime and Black Hole Thermodynamics},
  author={Wald, R.M.},
  isbn={9780226870274},
  lccn={94011065},
  series={Chicago Lectures in Physics},
  url={http://books.google.de/books?id=Iud7eyDxT1AC},
  year={1994},
  publisher={University of Chicago Press}
}
@book{greinerQED,
  title={Quantum Electrodynamics},
  author={Greiner, W. and Reinhardt, J.},
  isbn={9783540875611},
  lccn={2008937903},
  series={Physics and Astronomy},
  url={http://books.google.fr/books?id=5Kd3dBL8a64C},
  year={2008},
  publisher={Springer}
}
@book{hatano2011,
  title={Charged Particle and Photon Interactions with Matter: Recent Advances, Applications, and Interfaces},
  author={Hatano, Y. and Katsumura, Y. and Mozumder, A.},
  isbn={9781439811801},
  url={http://books.google.fr/books?id=Vj154iUYdmwC},
  year={2011},
  publisher={Taylor \& Francis}
}
@book{fulling,
  title={Aspects of Quantum Field Theory in Curved Spacetime},
  author={Fulling, S.A.},
  isbn={9780521377683},
  lccn={89211726},
  series={London Mathematical Society Student Texts},
  url={http://books.google.fr/books?id=Zo5\_3cmtFEUC},
  year={1989},
  publisher={Cambridge University Press}
}
@book{jackson1999,
  title={Classical Electrodynamics},
  author={Jackson, J.D.},
  isbn={9780471309321},
  lccn={97046873},
  url={http://books.google.fr/books?id=GuYNngEACAAJ},
  year={1999},
  publisher={Wiley}
}
@book{sakurai2006,
  title={Advanced Quantum Mechanics},
  author={Sakurai, J.J.},
  isbn={9788177589160},
  url={http://books.google.fr/books?id=lvmSZkzDFt0C},
  year={2006},
  publisher={Pearson Education, Incorporated}
}
@book{cornwell1984vol2,
  title={Group theory in physics},
  author={Cornwell, J.F.},
  number={vol.~2},
  isbn={9780121898021},
  lccn={83072256},
  series={Techniques of physics},
  url={http://books.google.fr/books?id=bKQ7AQAAIAAJ},
  year={1984},
  publisher={Academic Press}
}
@book{scharf,
  title={Finite Quantum Electrodynamics: The Causal Approach, Third Edition},
  author={Scharf, G.},
  isbn={9780486782287},
  series={Dover Books on Physics},
  url={http://books.google.co.uk/books?id=N3lpAwAAQBAJ},
  year={2014},
  publisher={Dover Publications}
}
@book{nagashima,
  title={Elementary Particle Physics: Foundations of the Standard Model},
  author={Nagashima, Y.},
  number={v. 2},
  isbn={9783527648900},
  url={https://books.google.co.uk/books?id=QYlX6AL4CtwC},
  year={2013},
  publisher={Wiley}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ARTICLE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@article{walterUni,
  title = {On the Kohn-Sham Approach to Time-Dependent
  Problems in a Density-Functional Framework},
  author = {Maitra, Neepa T. and van Leeuwen, Robert and Burke, Kieron},
  url = {arXiv:1506.04602}
}
@article{neepa2008,
  title = {Comment on ``Critique of the foundations of time-dependent density-functional theory''},
  author = {Maitra, Neepa T. and van Leeuwen, Robert and Burke, Kieron},
  journal = {Phys. Rev. A},
  volume = {78},
  issue = {5},
  pages = {056501},
  numpages = {4},
  year = {2008},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.78.056501},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.78.056501}
}

@article{rmb,
  title = {Time-dependent Kohn-Sham approach to quantum electrodynamics},
  author = {Ruggenthaler, M. and Mackenroth, F. and Bauer, D.},
  journal = {Phys. Rev. A},
  volume = {84},
  issue = {4},
  pages = {042107},
  numpages = {7},
  year = {2011},
  month = {Oct},
  doi = {10.1103/PhysRevA.84.042107},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.84.042107},
  publisher = {American Physical Society}
}
@article{furry1951,
  title = {On Bound States and Scattering in Positron Theory},
  author = {Furry, W. H.},
  journal = {Phys. Rev.},
  volume = {81},
  issue = {1},
  pages = {115--124},
  numpages = {0},
  year = {1951},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.81.115},
  url = {http://link.aps.org/doi/10.1103/PhysRev.81.115}
}
@article{RevModPhys.81.109,
  title = {The electronic properties of graphene},
  author = {Castro Neto, A. H. and Guinea, F. and Peres, N. M. R. and Novoselov, K. S. and Geim, A. K.},
  journal = {Rev. Mod. Phys.},
  volume = {81},
  issue = {1},
  pages = {109--162},
  year = {2009},
  month = {Jan},
  doi = {10.1103/RevModPhys.81.109},
  url = {http://link.aps.org/doi/10.1103/RevModPhys.81.109},
  publisher = {American Physical Society}
}
@article{macdonald1983,
  author={A H MacDonald},
  title={Spin-polarised relativistic exchange energies and potentials},
  journal={Journal of Physics C: Solid State Physics},
  volume={16},
  number={20},
  pages={3869},
  url={http://stacks.iop.org/0022-3719/16/i=20/a=012},
  year={1983},
  abstract={Expressions for the exchange energy of a relativistic polarised electron gas have been derived. These expressions have been evaluated numerically over a wide range of densities and polarisations. The leading-order relativistic corrections for the transverse exchange energy, which are of most importance in practice, have been evaluated analytically. The numerical results have been fitted to a simple form, suggested by the analytic leading-order-correction expressions, which should be useful for local-density-approximation applications.}
}
@article{xu1984,
  author={Bu Xing Xu and A K Rajagopal and M V Ramana},
  title={Theory of spin-polarised inhomogeneous relativistic electron systems. II},
  journal={Journal of Physics C: Solid State Physics},
  volume={17},
  number={8},
  pages={1339},
  url={http://stacks.iop.org/0022-3719/17/i=8/a=009},
  year={1984},
  abstract={A critical comparison of the authors earlier theory with a recent alternative theory of MacDonald (see ibid., vol.16, p.3896, 1983) is given. After correcting some errors in the previous work, new analytical results are presented here. Most importantly, it is pointed out that the authors theory is renormalisable and relativistically invariant in contrast to MacDonald's theory. His results for the leading-order relativistic parameter are the same as the authors present results since he did not use his theory in this regime. The physical picture associated with the theory of spin polarisation in a relativistic theory is spelled out in greater detail than before. It is found that the total exchange energy and the exchange potential change sign for different sets of values of the relativistic and magnetisation parameters.}
}
@article{raja1979,
  author={M V Ramana and A K Rajagopal},
  title={Relativistic spin-polarised electron gas},
  journal={Journal of Physics C: Solid State Physics},
  volume={12},
  number={22},
  pages={L845},
  url={http://stacks.iop.org/0022-3719/12/i=22/a=005},
  year={1979},
  abstract={The authors present a relativistic generalisation of the Bloch theory of a magnetic electron gas. It is shown that states of uniform magnetisation, as in the non-relativistic theory, do not appear as ground states in the Hartree-Fock approximation including transverse photon contributions. The exchange energy changes sign for certain values of the relativistic parameter ( beta =h(cross)k F /mc) and magnetisation so that spiral spin arrangements may be favoured.}
}
@article{raja1981,
  author={M V Ramana and A K Rajagopal},
  title={Theory of spin polarised inhomogeneous relativistic electron gas},
  journal={Journal of Physics C: Solid State Physics},
  volume={14},
  number={29},
  pages={4291},
  url={http://stacks.iop.org/0022-3719/14/i=29/a=016},
  year={1981},
  abstract={Describes a relativistic generalisation of the spin density functional formalism. The full Feynman propagator is presented and discussed. Effective single-particle Dirac equations for the polarised gas are given. Effective one-particle potentials for the magnetised gas are calculated in the local density scheme. These results are displayed graphically and their significance discussed.}
}
@article{brouder2002,
    author={Brouder, Christian},
    title={Renormalization of QED in an external field},
    journal={EPJ direct},
    volume={4},
    number={1},
    year={2002},
    url={http://dx.doi.org/10.1007/s1010502c0003},
    doi={10.1007/s1010502c0003},
    publisher={Springer-Verlag},
    keywords={12.20.-m; 11.10.Gh},
    pages={1-45},
    language={English}
}
@article{vanL1999,
  title = {Mapping from Densities to Potentials in Time-Dependent Density-Functional Theory},
  author = {van Leeuwen, Robert},
  journal = {Phys. Rev. Lett.},
  volume = {82},
  issue = {19},
  pages = {3863--3866},
  year = {1999},
  month = {May},
  doi = {10.1103/PhysRevLett.82.3863},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.82.3863},
  publisher = {American Physical Society}
}
@article{hawton1999a,
  title = {Photon position operator with commuting components},
  author = {Hawton, Margaret},
  journal = {Phys. Rev. A},
  volume = {59},
  issue = {2},
  pages = {954--959},
  year = {1999},
  month = {Feb},
  doi = {10.1103/PhysRevA.59.954},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.59.954},
  publisher = {American Physical Society}
}
@article{hawton1999b,
  title = {Photon wave functions in a localized coordinate space basis},
  author = {Hawton, Margaret},
  journal = {Phys. Rev. A},
  volume = {59},
  issue = {5},
  pages = {3223--3227},
  year = {1999},
  month = {May},
  doi = {10.1103/PhysRevA.59.3223},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.59.3223},
  publisher = {American Physical Society}
}
@article{hawton2010a,
  title = {Photon position measure},
  author = {Hawton, Margaret},
  journal = {Phys. Rev. A},
  volume = {82},
  issue = {1},
  pages = {012117},
  numpages = {6},
  year = {2010},
  month = {Jul},
  doi = {10.1103/PhysRevA.82.012117},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.82.012117},
  publisher = {American Physical Society}
}
@article{hawton2011,
  author={Margaret Hawton},
  title={Photon location in spacetime},
  journal={Physica Scripta},
  volume={2012},
  number={T147},
  pages={014014},
  url={http://stacks.iop.org/1402-4896/2012/i=T147/a=014014},
  year={2012},
  abstract={The Newton–Wigner basis of orthonormal localized states is generalized to orthonormal and relativistic biorthonormal bases on an arbitrary hyperplane in spacetime. This covariant formalism is applied to the measurement of photon location using a hypothetical three-dimensional (3D) array with pixels throughout space turned on at a fixed time and a timelike 2D photon counting array detector with good time resolution. A moving observer will see these detector arrays as rotated in spacetime but the spacelike and timelike experiments remain distinct.}
}
@article{hawton2013,
  title = {Photon counting by inertial and accelerated detectors},
  author = {Hawton, Margaret},
  journal = {Phys. Rev. A},
  volume = {87},
  issue = {4},
  pages = {042116},
  numpages = {10},
  year = {2013},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.87.042116},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.87.042116}
}
@article{hawton1995,
  title = {Photon number density operator  \textit{i}   \textbf{E}    $\cdot$      \textbf{A}},
  author = {Hawton, M. and Melde, T.},
  journal = {Phys. Rev. A},
  volume = {51},
  issue = {5},
  pages = {4186--4190},
  year = {1995},
  month = {May},
  doi = {10.1103/PhysRevA.51.4186},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.51.4186},
  publisher = {American Physical Society}
}
@article{keller2005,
title = "On the theory of spatial localization of photons ",
journal = "Physics Reports ",
volume = "411",
number = "1–3",
pages = "1 - 232",
year = "2005",
note = "",
issn = "0370-1573",
doi = "http://dx.doi.org/10.1016/j.physrep.2005.01.002",
url = "http://www.sciencedirect.com/science/article/pii/S0370157305000438",
author = "Ole Keller"
}
@article{lamb1995,
year={1995},
issn={0946-2171},
journal={Applied Physics B},
volume={60},
number={2-3},
doi={10.1007/BF01135846},
title={Anti-photon},
url={http://dx.doi.org/10.1007/BF01135846},
publisher={Springer-Verlag},
keywords={12.20.-m; 42.50.-p},
author={Lamb, W.E., Jr.},
pages={77-84},
language={English}
}
@article{chandra2012,
year={2012},
journal={Adv. Studies Theor. Phys.},
volume={6},
number={5-8},
title={Quantum mechanics of photons},
url={http://www.m-hikari.com/astp/astp2012/astp5-8-2012/chandrasekarASTP5-8-2012.pdf},
author={Chandrasekar, N.},
pages={391-397},
}
@article{BB1994,
year={1994},
journal={Acta Physica Polonica A},
volume={86},
number={97},
title={On the wave function of the photon},
url={http://www.cft.edu.pl/~birula/publ/APPPwf.pdf},
author={Bialynicki-Birula, I.},
}
@article{sipe1995,
  title = {Photon wave functions},
  author = {Sipe, J. E.},
  journal = {Phys. Rev. A},
  volume = {52},
  issue = {3},
  pages = {1875--1883},
  year = {1995},
  month = {Sep},
  doi = {10.1103/PhysRevA.52.1875},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.52.1875},
  publisher = {American Physical Society}
}
@article{vignale2004,
  title = {Mapping from current densities to vector potentials in time-dependent current density functional theory},
  author = {Vignale, Giovanni},
  journal = {Phys. Rev. B},
  volume = {70},
  issue = {20},
  pages = {201102},
  numpages = {4},
  year = {2004},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.70.201102},
  url = {http://link.aps.org/doi/10.1103/PhysRevB.70.201102}
}
@article{caban2013,
  title = {Spin operator in the Dirac theory},
  author = {Caban, Pawe\l{} and Rembieli\ifmmode \acute{n}\else \'{n}\fi{}ski, Jakub and W\l{}odarczyk, Marta},
  journal = {Phys. Rev. A},
  volume = {88},
  issue = {2},
  pages = {022119},
  numpages = {8},
  year = {2013},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.88.022119},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.88.022119}
}
@article{costella1995,
      author         = "Costella, John P. and McKellar, Bruce H.J.",
      title          = "{The Foldy-Wouthuysen transformation}",
      journal        = "Am.J.Phys.",
      volume         = "63",
      pages          = "1119",
      doi            = "10.1119/1.18017",
      year           = "1995",
      eprint         = "hep-ph/9503416",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UM-P-95-12, RCHEP-95-08",
      SLACcitation   = "%%CITATION = HEP-PH/9503416;%%",
}
@article{foldywoldy,
      author         = "Foldy, Leslie L. and Wouthuysen, Siegfried A.",
      title          = "{On the Dirac theory of spin 1/2 particle and its
                        nonrelativistic limit}",
      journal        = "Phys.Rev.",
      volume         = "78",
      pages          = "29-36",
      doi            = "10.1103/PhysRev.78.29",
      year           = "1950",
      SLACcitation   = "%%CITATION = PHRVA,78,29;%%",
}
@article{hilge1963,
title = "On the spin angular momentum of the Dirac particle ",
journal = "Nuclear Physics ",
volume = "40",
number = "0",
pages = "1 - 12",
year = "1963",
note = "",
issn = "0029-5582",
doi = "http://dx.doi.org/10.1016/0029-5582(63)90246-3",
url = "http://www.sciencedirect.com/science/article/pii/0029558263902463",
author = "J. Hilgevoord and S.A. Wouthuysen"
}
@article{ryder2001,
      author         = "Kirsch, Ingo and Ryder, Lewis H. and Hehl, Friedrich W.",
      title          = "{The Gordon decompositions of the inertial currents of
                        the Dirac electron correspond to a Foldy-Wouthuysen
                        transformation}",
      year           = "2001",
      eprint         = "hep-th/0102102",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = HEP-TH/0102102;%%",
}
@article{newtonwigner,
      author         = "Newton, T.D. and Wigner, Eugene P.",
      title          = "{Localized States for Elementary Systems}",
      journal        = "Rev.Mod.Phys.",
      volume         = "21",
      pages          = "400-406",
      doi            = "10.1103/RevModPhys.21.400",
      year           = "1949",
      SLACcitation   = "%%CITATION = RMPHA,21,400;%%",
}
@article{gorling2006,
  title = {Exact-Exchange Spin-Current Density-Functional Theory},
  author = {Rohra, Stefan and G\"orling, Andreas},
  journal = {Phys. Rev. Lett.},
  volume = {97},
  issue = {1},
  pages = {013005},
  numpages = {4},
  year = {2006},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.97.013005},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.97.013005}
}
@article{gordon1928,
year={1928},
issn={0044-3328},
journal={Zeitschrift für Physik},
volume={50},
number={9-10},
doi={10.1007/BF01327881},
title={Der Strom der Diracschen Elektronentheorie},
url={http://dx.doi.org/10.1007/BF01327881},
publisher={Springer-Verlag},
author={Gordon, W.},
pages={630-632},
language={German}
}
@article{vignale1987,
  title = {Density-functional theory in strong magnetic fields},
  author = {Vignale, G. and Rasolt, Mark},
  journal = {Phys. Rev. Lett.},
  volume = {59},
  issue = {20},
  pages = {2360--2363},
  numpages = {0},
  year = {1987},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.59.2360},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.59.2360}
}
@article{raja1994,
  title = {Time-dependent functional theory of coupled electron and electromagnetic fields in condensed-matter systems},
  author = {Rajagopal, A. K.},
  journal = {Phys. Rev. A},
  volume = {50},
  issue = {5},
  pages = {3759--3765},
  numpages = {0},
  year = {1994},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.50.3759},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.50.3759}
}
@article{ruij1977,
      author         = "Ruijsenaars, S.N.M.",
      title          = "{Charged Particles in External Fields. 2. The Quantized
                        Dirac and Klein-Gordon Theories}",
      journal        = "Commun.Math.Phys.",
      volume         = "52",
      pages          = "267",
      doi            = "10.1007/BF01609487",
      year           = "1977",
      reportNumber   = "Print-76-0424 (LEIDEN)",
      SLACcitation   = "%%CITATION = CMPHA,52,267;%%",
}
@article{deckert2009,
      author         = "Deckert, D.-A. and Durr, D. and Merkl, F. and
                        Schottenloher, M.",
      title          = "{Time Evolution of the External Field Problem in QED}",
      journal        = "J.Math.Phys.",
      volume         = "51",
      pages          = "122301",
      doi            = "10.1063/1.3506403",
      year           = "2010",
      eprint         = "0906.0046",
      archivePrefix  = "arXiv",
      primaryClass   = "math-ph",
      SLACcitation   = "%%CITATION = ARXIV:0906.0046;%%",
}
@article{marecki2003,
      author         = "Marecki, Piotr",
      title          = "{Quantum electrodynamics on background external fields}",
      year           = "2003",
      eprint         = "hep-th/0312304",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DESY-THESIS-2004-002",
      SLACcitation   = "%%CITATION = HEP-TH/0312304;%%",
}
@article{lazarovici2013,
      author         = "Lazarovici, Dustin",
      title          = "{Time Evolution in the external field problem of Quantum
                        Electrodynamics}",
      year           = "2013",
      eprint         = "1310.1778",
      archivePrefix  = "arXiv",
      primaryClass   = "math-ph",
      SLACcitation   = "%%CITATION = ARXIV:1310.1778;%%",
}
@article{haag1955,
      author         = "Haag, R.",
      title          = "{On quantum field theories}",
      journal        = "Kong.Dan.Vid.Sel.Mat.Fys.Med.",
      volume         = "29N12",
      pages          = "1-37",
      year           = "1955",
      reportNumber   = "CERN-55-08",
      SLACcitation   = "%%CITATION = KDVSA,29N12,1;%%",
}
@article{robert1999,
  title = {Mapping from Densities to Potentials in Time-Dependent Density-Functional Theory},
  author = {van Leeuwen, Robert},
  journal = {Phys. Rev. Lett.},
  volume = {82},
  issue = {19},
  pages = {3863--3866},
  numpages = {0},
  year = {1999},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.82.3863},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.82.3863}
}
@article{rungegross,
  title = {Density-Functional Theory for Time-Dependent Systems},
  author = {Runge, Erich and Gross, E. K. U.},
  journal = {Phys. Rev. Lett.},
  volume = {52},
  issue = {12},
  pages = {997--1000},
  numpages = {0},
  year = {1984},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.52.997},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.52.997}
}
@article{hohekohn,
  title = {Inhomogeneous Electron Gas},
  author = {Hohenberg, P. and Kohn, W.},
  journal = {Phys. Rev.},
  volume = {136},
  issue = {3B},
  pages = {B864--B871},
  numpages = {0},
  year = {1964},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.136.B864},
  url = {http://link.aps.org/doi/10.1103/PhysRev.136.B864}
}
@incollection{BB1996,
title = "V Photon Wave Function ",
editor = "E. Wolf",
booktitle = "",
publisher = "Elsevier",
year = "1996",
volume = "36",
pages = "245 - 294",
series = "Progress in Optics ",
issn = "0079-6638",
doi = "http://dx.doi.org/10.1016/S0079-6638(08)70316-0",
url = "http://www.sciencedirect.com/science/article/pii/S0079663808703160",
author = "Iwo Bialynicki-Birula"
}
@article{smith2007,
  author={Brian J Smith and M G Raymer},
  title={Photon wave functions, wave-packet quantization of light, and coherence theory},
  journal={New Journal of Physics},
  volume={9},
  number={11},
  pages={414},
  url={http://stacks.iop.org/1367-2630/9/i=11/a=414},
  year={2007},
}
@article{stewart1984,
  title = {Heavy-fermion systems},
  author = {Stewart, G. R.},
  journal = {Rev. Mod. Phys.},
  volume = {56},
  issue = {4},
  pages = {755--787},
  numpages = {0},
  year = {1984},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.56.755},
  url = {http://link.aps.org/doi/10.1103/RevModPhys.56.755}
}
@article{heisenberg1935,
      author         = "Heisenberg, W. and Euler, H.",
      title          = "{Consequences of Dirac's theory of positrons}",
      journal        = "Z.Phys.",
      volume         = "98",
      pages          = "714-732",
      doi            = "10.1007/BF01343663",
      year           = "1936",
      eprint         = "physics/0605038",
      archivePrefix  = "arXiv",
      primaryClass   = "physics",
      SLACcitation   = "%%CITATION = PHYSICS/0605038;%%",
}
@article{euler1935,
year={1935},
issn={0028-1042},
journal={Naturwissenschaften},
volume={23},
number={15},
doi={10.1007/BF01493898},
title={Über die Streuung von Licht an Licht nach der Diracschen Theorie},
url={http://dx.doi.org/10.1007/BF01493898},
publisher={Springer-Verlag},
author={Euler, H. and Kockel, B.},
pages={246-247},
language={German}
}
@article{dunne2012,
      author         = "Dunne, Gerald V.",
      title          = "{The Heisenberg-Euler Effective Action: 75 years on}",
      journal        = "Int.J.Mod.Phys.",
      volume         = "A27",
      pages          = "1260004",
      doi            = "10.1142/S2010194512007222, 10.1142/S0217751X12600044",
      year           = "2012",
      eprint         = "1202.1557",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1202.1557;%%",
}
@article{chandrasekar2012,
  title={Quantum mechanics of photons},
  author={Chandrasekar, N},
  journal={Adv. Studies Theor. Phys},
  volume={6},
  pages={391--397},
  year={2012}
}
@article{scharf1982,
      author         = "Scharf, G. and Seipp, H.P.",
      title          = "{CHARGED VACUUM, SPONTANEOUS POSITRON PRODUCTION AND ALL
                        THAT}",
      journal        = "Phys.Lett.",
      volume         = "B108",
      pages          = "196-198",
      doi            = "10.1016/0370-2693(82)91173-X",
      year           = "1982",
      SLACcitation   = "%%CITATION = PHLTA,B108,196;%%",
}
@article{greiner1977,
      author         = "Reinhardt, J. and Greiner, W.",
      title          = "{Quantum Electrodynamics of Strong Fields}",
      journal        = "Rept.Prog.Phys.",
      volume         = "40",
      pages          = "219-295",
      doi            = "10.1088/0034-4885/40/3/001",
      year           = "1977",
      SLACcitation   = "%%CITATION = RPPHA,40,219;%%",
}
@article{szpak2006,
      author         = "Szpak, Nikodem",
      title          = "{Spontaneous particle creation in time-dependent
                        overcritical fields}",
      journal        = "J.Phys.",
      volume         = "A41",
      pages          = "164059",
      doi            = "10.1088/1751-8113/41/16/164059",
      year           = "2008",
      eprint         = "hep-th/0604101",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = HEP-TH/0604101;%%",
}
@article{ruggerubio,
  title = {Quantum-electrodynamical density-functional theory: Bridging quantum optics and electronic-structure theory},
  author = {Ruggenthaler, Michael and Flick, Johannes and Pellegrini, Camilla and Appel, Heiko and Tokatly, Ilya V. and Rubio, Angel},
  journal = {Phys. Rev. A},
  volume = {90},
  issue = {1},
  pages = {012508},
  numpages = {26},
  year = {2014},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.90.012508},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.90.012508}
}
@article{neepa2002,
  title = {Memory in Time-Dependent Density Functional Theory},
  author = {Maitra, Neepa T. and Burke, Kieron and Woodward, Chris},
  journal = {Phys. Rev. Lett.},
  volume = {89},
  issue = {2},
  pages = {023002},
  numpages = {4},
  year = {2002},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.89.023002},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.89.023002}
}
@article{parker1971,
      author         = "Parker, L.",
      title          = "{Quantized fields and particle creation in expanding
                        universes. 2.}",
      journal        = "Phys.Rev.",
      volume         = "D3",
      pages          = "346-356",
      doi            = "10.1103/PhysRevD.3.346, 10.1103/PhysRevD.3.2546",
      year           = "1971",
      SLACcitation   = "%%CITATION = PHRVA,D3,346;%%",
}
@article{MLB08,
  title = {Comment on ``Critique of the foundations of time-dependent density-functional theory''},
  author = {Maitra, Neepa T. and van Leeuwen, Robert and Burke, Kieron},
  journal = {Phys. Rev. A},
  volume = {78},
  issue = {5},
  pages = {056501},
  numpages = {4},
  year = {2008},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.78.056501},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.78.056501}
}
@article{neepacausality,
  title = {Comment on ``Critique of the foundations of time-dependent density-functional theory''},
  author = {Maitra, Neepa T. and van Leeuwen, Robert and Burke, Kieron},
  journal = {Phys. Rev. A},
  volume = {78},
  issue = {5},
  pages = {056501},
  numpages = {4},
  year = {2008},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.78.056501},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.78.056501}
}
@article{sch,
  title = {Critique of the foundations of time-dependent density-functional theory},
  author = {Schirmer, J. and Dreuw, A.},
  journal = {Phys. Rev. A},
  volume = {75},
  issue = {2},
  pages = {022513},
  numpages = {16},
  year = {2007},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.75.022513},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.75.022513}
}
@article{vL1999,
  title = {Mapping from Densities to Potentials in Time-Dependent Density-Functional Theory},
  author = {van Leeuwen, Robert},
  journal = {Phys. Rev. Lett.},
  volume = {82},
  issue = {19},
  pages = {3863--3866},
  numpages = {0},
  year = {1999},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.82.3863},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.82.3863}
}

@article{rugge2,
  title = {Quantum-electrodynamical density-functional theory: Bridging quantum optics and electronic-structure theory},
  author = {Ruggenthaler, Michael and Flick, Johannes and Pellegrini, Camilla and Appel, Heiko and Tokatly, Ilya V. and Rubio, Angel},
  journal = {Phys. Rev. A},
  volume = {90},
  issue = {1},
  pages = {012508},
  numpages = {26},
  year = {2014},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.90.012508},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.90.012508}
}
@article{fixed,
  author={M. Ruggenthaler and R. van Leeuwen},
  title={Global fixed-point proof of time-dependent density-functional theory},
  journal={EPL (Europhysics Letters)},
  volume={95},
  number={1},
  pages={13001},
  url={http://stacks.iop.org/0295-5075/95/i=1/a=13001},
  year={2011}
}
@article{fuks2014b,
author ="Fuks, Johanna I. and Maitra, Neepa T.",
title  ="Challenging adiabatic time-dependent density functional theory with a Hubbard dimer: the case of time-resolved long-range charge transfer",
journal  ="Phys. Chem. Chem. Phys.",
year  ="2014",
volume  ="16",
issue  ="28",
pages  ="14504-14513",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C4CP00118D",
url  ="http://dx.doi.org/10.1039/C4CP00118D",
}
@article{fuks2013,
  title = {Time-dependent exchange-correlation functional for a Hubbard dimer: Quantifying nonadiabatic effects},
  author = {Fuks, Johanna I. and Farzanehpour, Mehdi and Tokatly, Ilya V. and Appel, Heiko and Kurth, Stefan and Rubio, Angel},
  journal = {Phys. Rev. A},
  volume = {88},
  issue = {6},
  pages = {062512},
  numpages = {7},
  year = {2013},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.88.062512},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.88.062512}
}
@article{fuks2014a,
  title = {Charge transfer in time-dependent density-functional theory: Insights from the asymmetric Hubbard dimer},
  author = {Fuks, J. I. and Maitra, N. T.},
  journal = {Phys. Rev. A},
  volume = {89},
  issue = {6},
  pages = {062502},
  numpages = {6},
  year = {2014},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.89.062502},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.89.062502}
}
@article{deckert2014,
      author         = "Deckert, D.-A. and Merkl, F.",
      title          = "{Dirac Equation with External Potential and Initial Data
                        on Cauchy Surfaces}",
      journal        = "J.Math.Phys.",
      volume         = "55",
      pages          = "122305",
      doi            = "10.1063/1.4902376",
      year           = "2014",
      eprint         = "1404.1401",
      archivePrefix  = "arXiv",
      primaryClass   = "math-ph",
      SLACcitation   = "%%CITATION = ARXIV:1404.1401;%%",
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% INBOOK %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@inbook{dunne2004,
author={Gerald V. Dunne},
title={Heisenberg-Euler Effective Lagrangians: Basics and Extensions},
booktitle={From Fields to Strings: Circumnavigating Theoretical Physics},
chapter={14},
pages={445-522},
URL={http://www.worldscientific.com/doi/abs/10.1142/9789812775344_0014},
eprint={http://www.worldscientific.com/doi/pdf/10.1142/9789812775344_0014},
doi={10.1142/9789812775344_0014}
}
@inbook{BB1996,
booktitle={Progress in Optics},
editor={Wolf, E.},
author={Bialynicki-Birula, Iwo},
number={v. 36},
year={1996},
publisher={Elsevier},
address={Amsterdam},
url={http://arxiv.org/abs/quant-ph/0508202}
}
@inbook{saari2011,
author = {Peeter Saari},
title = {Photon Localization Revisited},
booktitle = {Quantum Optics and Laser Experiments},
chapter = {3},
pages = {49-66},
doi = {10.5772/29895}
}
%URL = {http://www.intechopen.com/books/quantum-optics-and-laser-experiments/photon-localization-revisited},
%eprint = {http://www.intechopen.com/books/quantum-optics-and-laser-experiments/photon-localization-revisited}
%}

@article{wald2014,
      author         = "Hollands, Stefan and Wald, Robert M.",
      title          = "{Quantum fields in curved spacetime}",
      year           = "2014",
      eprint         = "1401.2026",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      SLACcitation   = "%%CITATION = ARXIV:1401.2026;%%",
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PhD THESIS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@article{mareckithesis,
      author         = "Marecki, Piotr",
      title          = "{Quantum electrodynamics on background external fields}",
      year           = "2003",
      eprint         = "hep-th/0312304",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DESY-THESIS-2004-002",
      SLACcitation   = "%%CITATION = HEP-TH/0312304;%%",
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% JKD ADDITIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@article{ghosh1988,
  title = {Density-functional theory of many-electron systems subjected to time-dependent electric and magnetic fields},
  author = {Ghosh, Swapan K. and Dhara, Asish K.},
  journal = {Phys. Rev. A},
  volume = {38},
  issue = {3},
  pages = {1149--1158},
  numpages = {0},
  year = {1988},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.38.1149},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.38.1149}
}
@article{capelle2001,
  title = {Spin Currents and Spin Dynamics in Time-Dependent Density-Functional Theory},
  author = {Capelle, K. and Vignale, G. and Gy\"orffy, B. L.},
  journal = {Phys. Rev. Lett.},
  volume = {87},
  issue = {20},
  pages = {206403},
  numpages = {4},
  year = {2001},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.87.206403},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.87.206403}
}
@article{yabana2012,
  title = {Time-dependent density functional theory for strong electromagnetic fields in crystalline solids},
  author = {Yabana, K. and Sugiyama, T. and Shinohara, Y. and Otobe, T. and Bertsch, G. F.},
  journal = {Phys. Rev. B},
  volume = {85},
  issue = {4},
  pages = {045134},
  numpages = {11},
  year = {2012},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.85.045134},
  url = {http://link.aps.org/doi/10.1103/PhysRevB.85.045134}
}
@article{chaix1989,
  author={Chaix, P. and Iracane, D.},
  title={From quantum electrodynamics to mean-field theory. I. The Bogoliubov-Dirac-Fock formalism},
  journal={Journal of Physics B: Atomic, Molecular and Optical Physics},
  volume={22},
  number={23},
  pages={3791},
  url={http://stacks.iop.org/0953-4075/22/i=23/a=004},
  year={1989}
}

@book{marques2006,
  added-at = {2009-09-09T17:55:18.000+0200},
  author = {Marques, Miguel A.L.},
  biburl = {http://www.bibsonomy.org/bibtex/2c3705dad58b0963198c8953036efb788/pbuczek},
  edition = {Berlin, Heidelberg},
  interhash = {d87942ab939127b28b0d690c52f05609},
  intrahash = {c3705dad58b0963198c8953036efb788},
  keywords = {imported},
  owner = {pbuczek},
  publisher = {Springer},
  series = {Lecture Notes in Physics},
  timestamp = {2009-09-09T17:55:18.000+0200},
  title = {Time-Dependent Density Functional Theory},
  url = {http://dx.doi.org/10.1007/b11767107},
  volume = 706,
  year = 2006
}

@article{haag1964,
  author   = {Haag, R. and Kastler, D.},
  doi      = {10.1063/1.1704187},
  journal  = {J. Math. Phys.},
  keywords = {Quantum field theory, Functional analysis, Mathematical physics},
  pages    = {848--861},
  title    = {An algebraic approach to quantum field theory},
  volume   = {5},
  year     = {1964}
}

@inproceedings{jaffe2000,
    address = {London},
    author = {Jaffe, A.},
    booktitle = {Mathematical Physics 2000},
    citeulike-article-id = {12411273},
    editor = {Fokas, A. and Grigoryan, A. and Kibble, T. and Zegarlinski, B.},
    keywords = {foundations, physics, qft, review},
    pages = {111--127},
    posted-at = {2013-06-12 16:12:14},
    priority = {0},
    publisher = {Imperial College Press},
    title = {Constructive Quantum Field Theory},
    year = {2000}
}
@article{capelle2001b,
  title = {Nonuniqueness of the Potentials of Spin-Density-Functional Theory},
  author = {Capelle, K. and Vignale, G.},
  journal = {Phys. Rev. Lett.},
  volume = {86},
  issue = {24},
  pages = {5546--5549},
  numpages = {0},
  year = {2001},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.86.5546},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.86.5546}
}
@article{oliveira1988,
  title = {Density-Functional Theory for Superconductors},
  author = {Oliveira, L. N. and Gross, E. K. U. and Kohn, W.},
  journal = {Phys. Rev. Lett.},
  volume = {60},
  issue = {23},
  pages = {2430--2433},
  numpages = {0},
  year = {1988},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.60.2430},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.60.2430}
}
@article{liang1998,
  title = {Pair Production by Ultraintense Lasers},
  author = {Liang, Edison P. and Wilks, Scott C. and Tabak, Max},
  journal = {Phys. Rev. Lett.},
  volume = {81},
  issue = {22},
  pages = {4887--4890},
  numpages = {0},
  year = {1998},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.81.4887},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.81.4887}
}

@article{bogoliubov1947,
  Author = {N. N. Bogoliubov},
  Date-Added = {2010-06-22 15:10:14 -0400},
  Date-Modified = {2010-07-26 13:48:52 -0400},
  Journal = {Journal of Physics (Moscow)},
  Keywords = {QFT, Bose gas},
  Number = {1},
  Pages = {23--32},
  Title = {On the theory of superfluidity},
  Volume = {11},
  Year = {1947}
}

@article{glauber1963,
  title = {Coherent and Incoherent States of the Radiation Field},
  author = {Glauber, Roy J.},
  journal = {Phys. Rev.},
  volume = {131},
  issue = {6},
  pages = {2766--2788},
  numpages = {0},
  year = {1963},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.131.2766},
  url = {http://link.aps.org/doi/10.1103/PhysRev.131.2766}
}

@article{tokatly2003,
  title = {Local exchange-correlation vector potential with memory in time-dependent density functional theory:$\hskip0.3em${}The generalized hydrodynamics approach},
  author = {Tokatly, I. V. and Pankratov, O.},
  journal = {Phys. Rev. B},
  volume = {67},
  issue = {20},
  pages = {201103},
  numpages = {4},
  year = {2003},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.67.201103},
  url = {http://link.aps.org/doi/10.1103/PhysRevB.67.201103}
}

@techreport{plimpton1993fast,
  title={Fast parallel algorithms for short-range molecular dynamics},
  author={Plimpton, Steve},
  year={1993},
  institution={Sandia National Labs., Albuquerque, NM (United States)}
}
@article{heinz2008accurate,
  title={Accurate simulation of surfaces and interfaces of face-centered cubic metals using 12- 6 and 9- 6 Lennard-Jones potentials},
  author={Heinz, Hendrik and Vaia, RA and Farmer, BL and Naik, RR},
  journal={The Journal of Physical Chemistry C},
  volume={112},
  number={44},
  pages={17281-17290},
  year={2008},
  publisher={ACS Publications}
}

@article{Namba_1970,
	doi = {10.1143/jjap.9.1326},
	url = {https://doi.org/10.1143/jjap.9.1326},
	year = 1970,
	month = {nov},
	publisher = {{IOP} Publishing},
	volume = {9},
	number = {11},
	pages = {1326--1329},
	author = {Yoshikatsu Namba},
	title = {Resistivity and Temperature Coefficient of Thin Metal Films with Rough Surface},
	journal = {Japanese Journal of Applied Physics},
}





